Identifying 3D Genome Organization in Diploid Organisms via Euclidean Distance Geometry

The spatial organization of the DNA in the cell nucleus plays an important role for gene regulation, DNA replication, and genomic integrity. Through the development of chromosome conformation capture experiments (such as 3C, 4C, Hi-C) it is now possible to obtain the contact frequencies of the DNA at the whole-genome level. In this paper, we study the problem of reconstructing the 3D organization of the genome from such whole-genome contact frequencies. A standard approach is to transform the contact frequencies into noisy distance measurements and then apply semidefinite programming (SDP) formulations to obtain the 3D configuration. However, neglected in such reconstructions is the fact that most eukaryotes including humans are diploid and therefore contain two copies of each genomic locus. We prove that the 3D organization of the DNA is not identifiable from distance measurements derived from contact frequencies in diploid organisms. In fact, there are infinitely many solutions even in the noise-free setting. We then discuss various additional biologically relevant and experimentally measurable constraints (including distances between neighboring genomic loci and higher-order interactions) and prove identifiability under these conditions. Furthermore, we provide SDP formulations for computing the 3D embedding of the DNA with these additional constraints and show that we can recover the true 3D embedding with high accuracy from both noiseless and noisy measurements. Finally, we apply our algorithm to real pairwise and higher-order contact frequency data and show that we can recover known genome organization patterns.

==> Identifying 3D Genome Organization in Diploid Organisms via Euclidean Distance Geometry arxiv/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
\DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
 \DeclareGraphicsExtensions{.eps}
\fi

% Add packages and commands (Begin Anastasiya)
% \usepackage{caption}
% \usepackage{subcaption}
%% Used in table and figure examples below
\usepackage{dsfont}
%\usepackage{pdfpages}
\usepackage[caption=false]{subfig}
\newcommand{\RP}{\mathbb{RP}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\xsi}{(x_n^*)^{(i)}}
\newcommand{\ysi}{(y_n^*)^{(i)}}
\newcommand{\xsone}{(x_n^*)^{(1)}}
\newcommand{\ysone}{(y_n^*)^{(1)}}
\newcommand{\xstwo}{(x_n^*)^{(2)}}
\newcommand{\ystwo}{(y_n^*)^{(2)}}
\newcommand{\xsit}{(x'_n)^{(i)}}
\newcommand{\ysit}{(y'_n)^{(i)}}
\newcommand{\xsonet}{(x'_n)^{(1)}}
\newcommand{\ysonet}{(y'_n)^{(1)}}
\newcommand{\xstwot}{(x'_n)^{(2)}}
\newcommand{\ystwot}{(y'_n)^{(2)}}
\newcommand{\xsitt}{(x''_n)^{(i)}}
\newcommand{\ysitt}{(y''_n)^{(i)}}
\newcommand{\xsonett}{(x''_n)^{(1)}}
\newcommand{\ysonett}{(y''_n)^{(1)}}
\newcommand{\xstwott}{(x''_n)^{(2)}}
\newcommand{\ystwott}{(y''_n)^{(2)}}
\newcommand{\xone}{x_n^{(1)}}
\newcommand{\yone}{y_n^{(1)}}
\newcommand{\xtwo}{x_n^{(2)}}
\newcommand{\ytwo}{y_n^{(2)}}
\newcommand{\xni}{x_n^{(i)}}
\newcommand{\yni}{y_n^{(i)}}
\newcommand{\xtildeone}{\widetilde{x}_n^{(1)}}
\newcommand{\ytildeone}{\widetilde{y}_n^{(1)}}
\newcommand{\xtildetwo}{\widetilde{x}_n^{(2)}}
\newcommand{\ytildetwo}{\widetilde{y}_n^{(2)}}
\newcommand{\xslast}{(x_n^*)^{(k+1)}}
\newcommand{\yslast}{(y_n^*)^{(k+1)}}
\newcommand{\Dsi}{(D_{n-2,n-1,n}^*)^{(i)}}

\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\logdet}{logdet}
\DeclareMathOperator*{\argmin}{argmin}
%%%% End Anastasiya %%%%%%%%%%

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{3D Genome Organization in Diploid Organisms}{A. Belyaeva, K. Kubjas, L. J. Sun and C. Uhler}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Identifying 3D Genome Organization in Diploid Organisms via Euclidean Distance Geometry\thanks{Submitted.
\funding{Anastasiya Belyaeva was supported by an NSF Graduate Research Fellowship
(1122374), the Abdul Latif Jameel World Water and Food Security Lab (J-WAFS) at MIT and the MIT J-Clinic for Machine Learning and Health. Kaie Kubjas was supported by the European Union's Horizon 2020 research and innovation programme: Marie Sk\l{}odowska-Curie grant agreement No. 748354, research carried out at LIDS, MIT and Team PolSys, LIP6, Sorbonne University. Caroline Uhler was partially supported by NSF (DMS-1651995), ONR (N00014-17-1-2147 and N00014-18-1-2765), IBM, and a Simons Investigator Award. 
}}}

% Authors: full names plus addresses.
\author{Anastasiya Belyaeva\thanks{Laboratory for Information and Decision Systems, Department of Electrical Engineering and Computer Science, and Institute for Data, Systems and Society, Massachusetts Institute of Technology, Cambridge, MA 
  (\email{belyaeva@mit.edu}, \email{sunl@mit.edu}, \email{cuhler@mit.edu}).}
\and Kaie Kubjas\thanks{Department of Mathematics and Systems Analysis, Aalto University, Espoo, Finland
  (\email{kaie.kubjas@aalto.fi}).}
\and Lawrence J. Sun\footnotemark[2]
%\thanks{Mountain View, CA 
%  (\email{ptfrank@fictional.edu}).
%}
\and Caroline Uhler\footnotemark[2].}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> Identifying 3D Genome Organization in Diploid Organisms via Euclidean Distance Geometry arxiv/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
